Semantic Support for Log Analysis of Safety-Critical Embedded Systems

Testing is a relevant activity for the development life-cycle of Safety Critical Embedded systems. In particular, much effort is spent for analysis and classification of test logs from SCADA subsystems, especially when failures occur. The human expertise is needful to understand the reasons of failures, for tracing back the errors, as well as to understand which requirements are affected by errors and which ones will be affected by eventual changes in the system design. Semantic techniques and full text search are used to support human experts for the analysis and classification of test logs, in order to speedup and improve the diagnosis phase. Moreover, retrieval of tests and requirements, which can be related to the current failure, is supported in order to allow the discovery of available alternatives and solutions for a better and faster investigation of the problem.

==> sections/casestudy_new.tex <==

\section{ERMTS SCADA  {\color{red} Alessio }}
\label{casestudy}
European railway's competitiveness. ETCS (European Train Control System) is an ERTMS basic component: it is an Automatic Train Protection system (ATP) to replace the existing national ATP-systems. UNISIG is an industrial consortium which was created to develop the ERTMS/ETCS technical specifications and actively contributes to the activities of the European Railway Agency in order to assure the \textit{interoperability} that is the main driver for ERTMS in the context of the European Railway Network. The meaning of interoperability is two-fold: on the one hand, it refers to a geographical interoperability between countries and projects (a train fitted with ERTMS may run on any other ERTMS-equipped line); on the other hand, it also refers to a technical notion of interoperability between suppliers (a train fitted by a given supplier will be able to run on any other trackside infrastructure installed by another supplier). This opens the supply market and increases competition within the industry. The ERTMS/
ETCS 
application has three levels that define different uses of ERTMS as a train control system, ranging from track to train communications (level 1) to continuous communications between the train and the Radio Block Centre (level 2). Level 3, which is in a conceptual phase, will further increase ERTMS’ potential by introducing a moving block technology. This Pilot Application (PA) deals with ERTMS level 1.
ERTMS level 1 is designed as an add-on to or overlays a conventional line already equipped with line side signals and train detection equipment which locates the train. ERTMS level 1 has two main subsystems:
\begin{itemize}
 \item Ground subsystem: collects and transmits track data (speed limitations, signal-status, etc.) to the on-board subsystem;
\item  On-board subsystem: analyzes data received from the ground and elaborates a safe speed profile.
\end{itemize}
Communication between the tracks and the train are ensured by dedicated balises (known as Eurobalises) located on the trackside adjacent to the line side signals at required intervals, and connected to the train control centre (Fig. \ref{ermts}). The balises contain pre-programmed track data. The train detection equipment sends the position of the train to the control centre. The control centre, which receives the position of all trains on the line, determines the new movement authority (MA) and sends it to the balise. Train passes over the balise, receiving the new movement authority and track data. The on-board computer then calculates its speed profile from the movement authority and the next braking point. This information is displayed to the driver. 
\begin{figure}[ht]
\centering
\includegraphics[width=2.5in]{img/ermts}
\caption{ERMTS Case Study}
\label{ermts}
\end{figure}
The industrial use case is a specific function of {\color{red} descrizione}\\
{\color{red} Descrivere il sistema in termini di SCADA}
\DIFaddbegin {\color {\DIFadd{blue}} \DIFadd{The ERTMS/ETCS systems presented need of equipment to address in a specific way the regulation and the supervisor of trains movement along the line in a centralized way, this is the SCADA (Supervisory Control and Data Acquisition) subsystem. Typically such subsystem have functionality for the remote control or automatic control, in order to allow a single operator to command different stations from one place,  to track trains and control railway signals, to set automatically routes and align the train ride to timetables; integrating and super visioning the entire network. 
Others functionality performed are the monitoring and the diagnosis of the state of the infrastructure through different kind of sensors and subsystems distributed along all the line (Passenger information, statistical data collection, etc.). 
Others functions are provided by the ATS (Automatic Train Supervision) and TMS (Traffic Management System) in conjunction with IXL (Interlocking) and ATC (Automatic Train Control )(nel caso sostituire con RBC). 
In particular the SCADA subsystem provide tool for automating planning and rooting optimization, monitoring of the traffic on the network in real time  and efficient platform allocation in station. Often the optimization about routing and platforms are static, based on pre-configured data, but in many cases the SCADA subsystem support operator decision, offering problems resolutions to optimization chooses based on dynamic data. The SCADA subsystem allow also the dispatching of commands towards the RBC, setting restriction on the line based on a particular state that could be unexpected or programmed , e.g. the TMS could send a restriction about the max speed to achieve in a section of the network due to a maintenance operations. The SCADA subsystem could receive also alarms from the network (warning lights or acoustic alarms) by one of the sensors or a subsystems, e.g. the RBC could give an alarm if the maximum possible number of trains present in line is reached.
The entire network could be divided in more supervisor nodes, with one or more operators., due to the big data of information presented to the operator and the effort of the management of this activities. In this situation the scada subsystem could have a hierarchic structure, with communication between nodes and messaging services exported to operators.
In order to have an idea of the large number of parameters to be monitored and analyzed by such system we can think that for a network of   middle high complexity there are 10000 object that can changes state in real time only concerning, the binary sections and the trains moving along the line. In addiction to this consider that the point controlled could be over 5000, over 3000 are the signaling object and around 1500 the text string used to communicate.}} 
\DIFaddend \subsection{A case study}

{\color{red} Alessio descrive come avviene il test e che tipi di log arrivano alla fine}
 \DIFaddbegin {\color {\DIFadd{blue}}   
\DIFadd{The test are written to cover the functional and configuration  specifications, based and compliant to normative. The test descriptions compose a set of behaviors of the system, a representation of the state of entities, signals and anomalies. In the test description there are also checks to be verified in order to declare the test passed, each test is repeated for each configurable and adaptable items present in line. All signaling items must be tested by the configuration test set. 
In order to reduce replication of test writing work for all configurable items for a particular functionality is used an abstract testing methodology as done for interlocking subsystem in }[\DIFadd{inserire articolo flammini}]\DIFadd{. An abstract test script is prepared based on the test description, but the reference to the involved control entities is symbolic, so the file is not executable and have to be instantiated with all possible related items.
In the first part of the script is declared the state of the system under test. These are a set of values carachterizing the railway network and the internal state of subsystem of interest. 
The other section of the test case is completed with an Input sequence and an output sequece. The input sequence is a list of stimuli sent to the system, they could be command sent by an operator to HMI subsystem or a change of status forced to simulate an anomaly behaviour of the system. Others changes of state could be due to the functions  exported by subsystems and not explicity declared by the test. The output sequence that is spaced out with the input instructions is a set of data or control actions which are produce by the system in response to a certain input sequence.
For each state, input sequence and output sequence are declared some checks to monitor easly the right execution of the test and in case of a detected error notify the failure to the test manager. The checks operate also as brack point, if the result of the test is False, the next item of the sequence (input or output) is not schedulated, the brack point are trasparent only to the control logic.
Applying the transformation Algorithm ad presented in }[] \DIFadd{for IXL, from the abstract test is obtained the configured test set, that could be executed in the testing environment.
(Parte in parte di aSTS, da trovare articolo da referenziare)
In order to automatize the test execution, a single test environment can take the entire set of scripts as input and execute them consecutively, reporting to a machine or directly to an user the log of the test and the result, including also a complete report about all the test executed from the test set. Note that test not executed due to different kind of problems are considered not passed test.
}

\DIFadd{Architettura  Ambiente di simulazione
Due to the issues described in section  }[] \DIFadd{these test are executed, until the robustness of the system is not guarantee, in laboratory in simulated environment first and with target subsystems then.
The environment used to execute the script produced is composed by a set of application software, each of them simulate the behavior of a particular subsystem. In presence of subsystems not influencing the execution of the test, they could be implemented in stimulated, in order to don't add worthless resource consumption or time and cost consumption due to development effort, always supplying the right stimuli. This software applications are interconnected by a middleware developed ad hoc in order to guarantee conditions near to real field as well as possible. 
Per migliorare le performance e raggiungere un buon throughput è installata un architettura ad hoc, I cuid dettagli verranno però tralasciati perchè non di interesse per questo lavoro (forse)
}\DIFaddend 


\DIFaddbegin \DIFadd{Log  di  output dell'esecuzione
The output of the test execution is a set of test logs that incude the report of test script execution, the monitor of all variables about simulated subsystems and the output of the stimulated one. The test script log is the script of the file executed in which are reported the timestamp of execution and the value assumed by variables to check. Therefore the test script contains the state, the input sequene as reported into the original file, but with the extension of the time stamp of execution. For what concerning the output sequence and the associated checks are reported the time stamp and respectively the value assumed by the output and in case of error the failure notification. Note that if a failure is detected the test is declared not passed and not others input or output items are processed. The report of the script executed is a simple way to verify the test result and the failure mode, but for an accurate analysis is essential to view what happen in each subsystems in order to understand the cause.
To make this activity is necessary to know the following kind of information: all the messages exchanges by the subsystems (e.g. the MA from RBC to train and the respective ack in response), all the state of entities installed in fields included the entities not monitored into the script(e.g the states of the switch point, all signals and track circuits), all internal variables of the subsystems object of the testing activities and the related output. Considering the big data amount, the number of changes for time unit and the different nature of the data, the monitoring and the reporting of variables is collected in different file,each of them divided for level of abstraction and macro function of interest.  }}
 \DIFaddend

==> sections/casestudy_old.tex <==

\section{ERMTS SCADA  {\color{red} Alessio }}
\label{casestudy}
European railway's competitiveness. ETCS (European Train Control System) is an ERTMS basic component: it is an Automatic Train Protection system (ATP) to replace the existing national ATP-systems. UNISIG is an industrial consortium which was created to develop the ERTMS/ETCS technical specifications and actively contributes to the activities of the European Railway Agency in order to assure the \textit{interoperability} that is the main driver for ERTMS in the context of the European Railway Network. The meaning of interoperability is two-fold: on the one hand, it refers to a geographical interoperability between countries and projects (a train fitted with ERTMS may run on any other ERTMS-equipped line); on the other hand, it also refers to a technical notion of interoperability between suppliers (a train fitted by a given supplier will be able to run on any other trackside infrastructure installed by another supplier). This opens the supply market and increases competition within the industry. The ERTMS/
ETCS 
application has three levels that define different uses of ERTMS as a train control system, ranging from track to train communications (level 1) to continuous communications between the train and the Radio Block Centre (level 2). Level 3, which is in a conceptual phase, will further increase ERTMS’ potential by introducing a moving block technology. This Pilot Application (PA) deals with ERTMS level 1.
ERTMS level 1 is designed as an add-on to or overlays a conventional line already equipped with line side signals and train detection equipment which locates the train. ERTMS level 1 has two main subsystems:
\begin{itemize}
 \item Ground subsystem: collects and transmits track data (speed limitations, signal-status, etc.) to the on-board subsystem;
\item  On-board subsystem: analyzes data received from the ground and elaborates a safe speed profile.
\end{itemize}
Communication between the tracks and the train are ensured by dedicated balises (known as Eurobalises) located on the trackside adjacent to the line side signals at required intervals, and connected to the train control centre (Fig. \ref{ermts}). The balises contain pre-programmed track data. The train detection equipment sends the position of the train to the control centre. The control centre, which receives the position of all trains on the line, determines the new movement authority (MA) and sends it to the balise. Train passes over the balise, receiving the new movement authority and track data. The on-board computer then calculates its speed profile from the movement authority and the next braking point. This information is displayed to the driver. 
\begin{figure}[ht]
\centering
\includegraphics[width=2.5in]{img/ermts}
\caption{ERMTS Case Study}
\label{ermts}
\end{figure}
The industrial use case is a specific function of {\color{red} descrizione}\\
{\color{red} Descrivere il sistema in termini di SCADA}
\subsection{A case study}

{\color{red} Alessio descrive come avviene il test e che tipi di log arrivano alla fine}



==> sections/proofconcept.tex <==
\section{Proof of Concept}
\begin{figure*}[ht]
\centering
\includegraphics[width=5in]{img/solr.png}
\caption{Document retrieval}
\label{solr}
\end{figure*}
When a new project is developed  it needs to define a new test plan from the requirements of that specific railway system. The test coverage must complain with all the requirements. The traceability matrix shows for each requirement the correspondent test(s). If some requirements are not covered, than it  needs to develop new tests or to motivate why they cannot be tested and to specify those activities  which can be used for demonstrate the compliance of the project.
Let us suppose the user is going to produce a test script from a specific test specification in order to fill the traceability matrix.
The test specification is a description of the state of signaling entities present in line (e.g. red signals), the action performed by the subsystem (e. g. the train) and behavior expected by the system (e. g. the ground system sends the MA to the train).
The following example explains a simple procedure describing the behavior of the train in response to some events occurring during the trip. The train must discard the telegram from the second $balise\_group$ and has to consider the last one due to the requirements about the linking information.

Let the test description being:\\
\textit{``The {\color{blue}\underline{train}} is located in the first {\color{blue}\underline{SBR}} and is using the {\color{blue}\underline{linking information}}. The {\color{blue}\underline{train capt}} the first {\color{blue}\underline{$balise\_group$}} present into the first {\color{blue}\underline{SBR}} and {\color{blue}\underline{receives}} the {\color{blue}\underline{MA}} till the {\color{blue}\underline{signal}} S3 at the end of the first {\color{blue}\underline{SBR}}. The {\color{blue}\underline{train}} moves through the second {\color{blue}\underline{SBR}} and {\color{blue}\underline{capt}} the new {\color{blue}\underline{$balise\_group$}}, not present into the {\color{blue}\underline{linking information list}}. The {\color{blue}\underline{OBU}} discards the {\color{blue}\underline{Telegram}} present into the {\color{blue}\underline{balise}} and moves ahead. The {\color{blue}\underline{train}} {\color{blue}\underline{capt}}  a third {\color{blue}\underline{$balise\_group$}}, marked as {\color{blue}\
underline{unlinked}}, reads the {\color{blue}\underline{telegram}} and updates the {\color{blue}\underline{MA}}[......]''.}

Our tool allow to the user the upload of the test description. All the elements from the ontology, which occur in the text,  are recognized and underlined. %as it is shown in Figure \ref{}.

Several option are available to the user. He could start from navigating the ontology browser shown in Figure \ref{jtree}. He can search for some terms in the text field. Or he can paste the text into the web page for automatic tagging of recognized terms. In the last case it is simple to set the root of the ontology tree with the concept of interest, or to check those concepts which are relevant for a text search within the document store.
Technically user actions start SPARQL queries described in Section \ref{sparql}  which aim at searching  the matching entities of the ontologies, searching relations between matching concepts and  listing subtypes or super-types of matching entities. All the obtained results can be effectively used to expand text queries to the Apache Solr document store.

Let us suppose that the user is interested in \textit{OBU},  \textit{linking information} and asks about any relations between them. It gets some triples and selects the following one: $(OBU, use, linking information)$.
The user is looking for all test documents which concern such expression, bit he wants also to expand the search
to those documents where the similar expressions occur with other concepts  equivalent to $OBU$.
Hence the system will replace $OBU$ with on-board equipment, SSB, ERTMS-ETCS on-board equipment.
Finally the SOLR back-end is queried using the following  triples 
 (SSB, use, linking information), (OBU, use, linking information), (on-board equippemnt, use, linking information), (ERTMS.ETCS on-board equipment, use, linking information).
 
 In this case the test scripts shown in Table \ref{reqs} are retrieved and the user can choose those which will be included into the traceability matrix, eventually marked for review if someone is affected by an  incoherence between the test and the current requirement.


==> sections/tool_old.tex <==
\section{A semantic support for log analysis}
\label{tool}
A semantic support for the user is provided by a web tool that is able to retrieve:
\begin{itemize}
 \item  requirements that are covered  by a specific test or test-set;
 \item  entities of the ontologies from a test description or from a requirement;
 \item  requirements and test descriptions related to a specified ontology item according to pre-defined reasoning inference rules;
 \item  the group of requirements and test descriptions which  share the same semantic.
\end{itemize}

In Figure \ref{arch1} the architecture of our tool is shown. On the left the user is able to browse the domain ontology and to trigger semantic reasoning by a friendly web interface. It also  provides  a form for searching documents by keywords. The keyword base query is expanded by a semantic engine. The semantic engine and the search engine are completely decoupled. The first one works on-line with synchronous requests. The second one works in batch mode to perform text analysis and in interactive mode to process  search requests.
\begin{figure}[ht]
\centering
includegraphics[width=3in,natwidth=804,natheight=622]{img/architecture.png} 
\caption{Architecture}
\label{arch1}
\end{figure}
\subsection{Ontology design}
The railway ontology has been developed for the current case study. It represents the knowledge about this specific domain through a set of concepts described in a structured dictionary  consisting of classes, relations, data properties and individuals.  
Classes (Entities) are entities that recur into the railway application. They can be both physical and abstract. e.g. the signaling equipment installed on the railway track (balise group), or the distance before a signal before which it needs to react.
Relations   describe  logical connection between  two entities of the railway domain. The relations  describe something that  an entities has or something that an entity is. For example the entity \textit{balise} is linked with property \textit{contain} to \textit{Telegram}. It means that  in a signaling entity of type balise  a Telegram is stored.
Axioms describe elementary relations, such as the sub-class between concepts or the equivalence.
Going deeply the class entities are divided into twelve main classes. 
Some of the follow.
\begin{itemize}
\item \textit{Action}:represents an  activity performed by an entity.  It produces a change of the status and/or a response of the system.
\item \textit{Capability}: describes a  function provided by a component of the system.
\item \textit{Event}: represents a set of external conditions or inputs. On their occurrence an action is triggered.
\item \textit{Operational} condition: define all the mode under which the railway system can perform his mission. 
\item \textit{Parameter}: includes all the parameters characterizing the state of the system, on the basis of which an operational condition can occur.
\item \textit{User}: represents the stakeholders of the railway domain. In order to consider all the safety  issues it needs to consider  the operators and the external subsystems that have a functional role in the system mission, but also  the customer of the railway infrastructure, who  could deviate the nominal behavior of the system.
\end{itemize}
In the Figure \ref{ontology1}  part of the ontology developed is presented.
\begin{figure*}[ht]
\centering
\includegraphics[width=5in]{img/ontology1.jpg}
\caption{Railway Ontology}
\label{ontology1}
\end{figure*}
The extract shown in Figure \ref{ontology1} focuses on the class \textit{Balise Group}, that is a real signaling entity installed along the line. This entity is composed by one or more transponders  \textit{Balise}, which have stored inside a set of information about the line properties. Information is communicated to the On Board Unit (\textit{SSB}) of the train through a \textit{Telegram}. All these information are represented into the picture as a graph where class are drawn as rectangle and relations and axioms between them by edges. Different kinds of edges mean different type of relations. The arch between \textit{Balise Group} and \textit{Balise} represents a \textit{Contain} relation. The same occurs between Balise and Telegram. The arch between \textit{SSB} and \textit{Balise} means that the train subsystem can \textit{Capt} the balise transponder.
The ontology has been written according to the W3C OWL-RDFS (Ontology Web Language - Resource Description Framework) standard. It is a   knowledge representation language widely used to describe web information. It is a set of triples. 
%The RDF construct are RDFS classes, associated properties and utility properties.
%In the picture below are reported a fragment of RDF code about the declaration of class \textit{Balise}. Subclass of Entity with the properties contain with values only in the domain indicated by the RDF resource Telegram.
% \begin{figure*}[h]
% \centering
% \includegraphics[width=5in]{img/ontology2.png}
% \caption{RDF view of Railway Ontology}
% \label{ontology2}
% \end{figure*}
\subsection{User interaction ad semantic reasoning}
For supporting ontology browsing and semantic reasoning we used jOWL.  jOWL is a jQuery plugin for navigation and visualization of OWL-RDFS documents. Moreover it provides APIs for SPARQL\_DL query.
SPARQL is a language for  semantic querying of a knowledge base
\begin{figure}[h]
\centering
\includegraphics[width=3.5in]{img/jtree.png}
\caption{Ontology browser}
\label{jtree}
\end{figure}
A number of SPARQL queries are supported natively by the jOWL library. Some examples are:
\begin{itemize}
 \item $Class(?a)$. It  can be used to list all the Classes of the ontology or to check if a given term is a Class of the ontology.
\item  $Type(?a, ?b)$. It allows to gets the Class if the individual ?b is given, or all the individuals belonging to the Class ?a.
\item $PropertyValue(?a, ?b, ?c)$. It returns all the properties and the correspondent values if the individual ?a is given. 
\end{itemize}
\begin{figure}[h]
\centering
\includegraphics[width=3.5in]{img/sparql.png}
\caption{Sparql queries}
\label{sparql}
\end{figure}

% Our query go in the etcs a will find the subtype of etcs, for each subtype of etcs found into the ontologies e.g. type R, the tool will find all requirements that involved the specific etcs (where performig a som), the user looking at the selected requirements could make better its configuration chose for the test script.
%  Pseudocode:
%  \begin{itemize}
%   \item take all entities present into the test description
% \item take all entities wth relation hasSubtype or has Type o which the entities of the test is the element ?a
% \item for each entity found search into requirements which could be involved
% \item group the requirements sorting by tag
% \item make the choose easier
%  \end{itemize}
\subsection{Text based processing}
For document analysis and indexing we used Apache Solr. $Solr^{TM}$ is a fast open source enterprise search platform from the Apache Lucene$^{TM}$ project. Its major features include powerful full-text search, hit highlighting, faceted search, near real-time indexing, dynamic clustering, database integration, rich document (e.g., Word, PDF) handling, and geospatial search. Solr is written in Java and runs as a standalone full-text search server within a servlet container such as Jetty. Solr uses the Lucene Java search library at its core for full-text indexing and search, and has REST-like HTTP/XML and JSON APIs.
Searches are done via HTTP GET on the select URL with the query string in the q parameter. You can pass a number of optional request parameters to the request handler to control what information is returned.\\
$q=video\&fl=name,id$ returns only $name$ and id $fields$ of the documents containing the  keyword ``video''. 

Faceted search takes the documents matched by a query and generates counts for various properties or categories. Links are usually provided that allows users to "drill down" or refine their search results based on the returned categories.
The following example searches for all documents (*:*) and requests counts by the category field cat:\\
$...\&q=*:*\&facet=true\&facet.field=cat$

\subsection{Big Data storage}
 
Graph databases \cite{graph} may overcome these  limitation of the as they   generally provide ACID transactions.

Neo4j\cite{neo}, is an open source, robust (fully ACID) transactional property graph database. Due to its graph data model, Neo4j is highly agile and blazing fast. For connected data operations, Neo4j runs a thousand times faster than relational databases. Nodes store data and edges represent relationships. The data model is called property graph to indicate that edges could have properties. Neo4j provides a REST interface or a Java API. The core engine of Neo4j supports the property graph model. This model can easily be adapted to support the LinkedData RDF model, consisting of Triples. Besides it is possible to add spatial indexes to already located data, and perform spatial operations on the data like searching for data within specified regions or within a specified distance of a point of interest. In addition classes are provided to expose the data to geotools and thereby to geotools enabled applications like geoserver and uDig.
% 
% \textbf{AllegroGraph} \cite{allegro} is a modern, high-performance, persistent graph database. AllegroGraph uses efficient memory utilization in combination with disk-based storage, enabling it to scale to billions of quads while maintaining superior performance. AllegroGraph supports SPARQL, RDFS++, and Prolog reasoning from numerous client applications. AllegroGraph is a proprietary product of Franz Inc., which markets a number of Semantic Web products and claims Pfizer, Ford, Kodak, NASA and the Department of Defense among its AllegroGraph customers.
% 
% \textbf{InfiniteGraph} \cite{infinite} InfiniteGraph is a proprietary graph database currently available in both free and paid license versions produced by Objectivity, a company that develops data technologies supporting large-scale, distributed data management, object persistence and relationship analytics. Its goal is to create a graph database with "virtually unlimited scalability." InfiniteGraph is used in applications including real-time and location-aware web and mobile advertising platforms, military operations planning and mission assurance, and advanced healthcare and patient records management.

Adoption of Neo4j will  provide custom API's and Query Languages and many support the W3C's RDF standard, including a SPARQL engine.  This model can easily integrated with the JoWL base front-end. 
Besides it is possible to add spatial indexes to already located data, and perform spatial operations on the data like searching for data within specified regions or within a specified distance of a point of interest. In addition classes are provided to expose the data to geotools and thereby to geotools enabled applications like geoservers.
% An example of a floating figure using the graphicx package.
% Note that \label must occur AFTER (or within) \caption.
% For figures, \caption should occur after the \includegraphics.
% Note that IEEEtran v1.7 and later has special internal code that
% is designed to preserve the operation of \label within \caption
% even when the captionsoff option is in effect. However, because
% of issues like this, it may be the safest practice to put all your
% \label just after \caption rather than within \caption{}.
%
% Reminder: the "draftcls" or "draftclsnofoot", not "draft", class
% option should be used if it is desired that the figures are to be
% displayed while in draft mode.
%
%\begin{figure}[!t]
%\centering
%\includegraphics[width=2.5in]{myfigure}
% where an .eps filename suffix will be assumed under latex, 
% and a .pdf suffix will be assumed for pdflatex; or what has been declared
% via \DeclareGraphicsExtensions.
%\caption{Simulation Results}
%\label{fig_sim}
%\end{figure}

% Note that IEEE typically puts floats only at the top, even when this
% results in a large percentage of a column being occupied by floats.


% An example of a double column floating figure using two subfigures.
% (The subfig.sty package must be loaded for this to work.)
% The subfigure \label commands are set within each subfloat command, the
% \label for the overall figure must come after \caption.
% \hfil must be used as a separator to get equal spacing.
% The subfigure.sty package works much the same way, except \subfigure is
% used instead of \subfloat.
%
%\begin{figure*}[!t]
%\centerline{\subfloat[Case I]\includegraphics[width=2.5in]{subfigcase1}%
%\label{fig_first_case}}
%\hfil
%\subfloat[Case II]{\includegraphics[width=2.5in]{subfigcase2}%
%\label{fig_second_case}}}
%\caption{Simulation results}
%\label{fig_sim}
%\end{figure*}
%
% Note that often IEEE papers with subfigures do not employ subfigure
% captions (using the optional argument to \subfloat), but instead will
% reference/describe all of them (a), (b), etc., within the main caption.


% An example of a floating table. Note that, for IEEE style tables, the 
% \caption command should come BEFORE the table. Table text will default to
% \footnotesize as IEEE normally uses this smaller font for tables.
% The \label must come after \caption as always.
%
%\begin{table}[!t]
%% increase table row spacing, adjust to taste
%\renewcommand{\arraystretch}{1.3}
% if using array.sty, it might be a good idea to tweak the value of
% \extrarowheight as needed to properly center the text within the cells
%\caption{An Example of a Table}
%\label{table_example}
%\centering
%% Some packages, such as MDW tools, offer better commands for making tables
%% than the plain LaTeX2e tabular which is used here.
%\begin{tabular}{|c||c|}
%\hline
%One & Two\\
%\hline
%Three & Four\\
%\hline
%\end{tabular}
%\end{table}


% Note that IEEE does not put floats in the very first column - or typically
% anywhere on the first page for that matter. Also, in-text middle ("here")
% positioning is not used. Most IEEE journals/conferences use top floats
% exclusively. Note that, LaTeX2e, unlike IEEE journals/conferences, places
% footnotes above bottom floats. This can be corrected via the \fnbelowfloat
% command of the stfloats package.


